Ensemble Deep Learning on Large, Mixed-Site fMRI Datasets in Autism and Other Tasks

Deep learning models for MRI classification face two recurring problems: they are typically limited by low sample size, and are abstracted by their own complexity (the "black box problem"). In this paper, we train a convolutional neural network (CNN) with the largest multi-source, functional MRI (fMRI) connectomic dataset ever compiled, consisting of 43,858 datapoints. We apply this model to a cross-sectional comparison of autism (ASD) vs typically developing (TD) controls that has proved difficult to characterise with inferential statistics. To contextualise these findings, we additionally perform classifications of gender and task vs rest. Employing class-balancing to build a training set, we trained 3$\times$300 modified CNNs in an ensemble model to classify fMRI connectivity matrices with overall AUROCs of 0.6774, 0.7680, and 0.9222 for ASD vs TD, gender, and task vs rest, respectively. Additionally, we aim to address the black box problem in this context using two visualization methods. First, class activation maps show which functional connections of the brain our models focus on when performing classification. Second, by analyzing maximal activations of the hidden layers, we were also able to explore how the model organizes a large and mixed-centre dataset, finding that it dedicates specific areas of its hidden layers to processing different covariates of data (depending on the independent variable analyzed), and other areas to mix data from different sources. Our study finds that deep learning models that distinguish ASD from TD controls focus broadly on temporal and cerebellar connections, with a particularly high focus on the right caudate nucleus and paracentral sulcus.

==> IJNS Submission (3)/figures/asd_or_not_fig.tex <==
\begin{figure*}
\centering
\raisebox{40ex}{\fontfamily{qhv}{\fontsize{30}{100}{\textbf{A}}}}
\includegraphics[width=0.6\linewidth]{images/wc_all_asd_or_not_top_100_collection_random.png}
\raisebox{40ex}{\fontfamily{qhv}{\fontsize{30}{100}{\textbf{B}}}}\includegraphics[width=0.45\linewidth]{images/diversity_index_covars_asd_or_not.png}
\raisebox{40ex}{\fontfamily{qhv}{\fontsize{30}{100}{\textbf{C}}}}\includegraphics[width=0.40\linewidth]{images/asd_or_not_auroc_plot.png}
\caption{Results for autism classification. (A) The 100 strongest connections of the mean class activation maps, with the maximum value taken across wavelet correlations. (B) The distribution of the diversity index of maximal activations across all filters over 300 models, showing how much filters in general were dedicated to particular phenotypes. (C) The overall classification AUROC and the AUROC of individual data collections in the model, showing the overall and relative success of the model.}
\label{fig:asd_or_not_fig}
\end{figure*}

==> IJNS Submission (3)/figures/collection_distributions.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=0.9\linewidth]{images/all_collection_dist.png}
\caption{The effects of collection-based class balancing on the total degree distributions of wavelet correlation matrices. Note that data is re-scaled to have values in between 0 and 1, and the distributions are normalized for comparisons to have a total area of 1.}
\label{fig:collection_distribution}
\end{center}
\end{figure*}

==> IJNS Submission (3)/figures/gender_fig.tex <==
\begin{figure*}
\centering
\raisebox{40ex}{\fontfamily{qhv}{\fontsize{30}{100}{\textbf{A}}}}
\includegraphics[width=0.6\linewidth]{images/wc_all_gender_top_100_collection_random.png}
\raisebox{40ex}{\fontfamily{qhv}{\fontsize{30}{100}{\textbf{B}}}}\includegraphics[width=0.45\linewidth]{images/diversity_index_covars_gender.png}
\raisebox{40ex}{\fontfamily{qhv}{\fontsize{30}{100}{\textbf{C}}}}\includegraphics[width=0.40\linewidth]{images/gender_auroc_plot.png}
\caption{Results for gender classification. (A) The 100 strongest connections of the mean class activation maps, with the maximum value taken across wavelet correlations. (B) The distribution of the diversity index of maximal activations across all filters over 300 models, showing how much filters in general were dedicated to particular phenotypes. (C) The overall classification AUROC and the AUROC of individual data collections in the model, showing the overall and relative success of the model.}
\label{fig:gender_fig}
\end{figure*}

==> IJNS Submission (3)/figures/histogram_accs.tex <==
\begin{figurehere}
\centering
%\includegraphics[width=0.9\columnwidth]{images/cross_accs_histogram.png}
\includegraphics[width=0.9\columnwidth]{images/cross_aurocs_histogram.png}
\caption{Histograms of all AUROCS for 300 independent models, using different, stratified samples of the whole dataset.}
\label{fig:histogram_accs}
\end{figurehere}

==> IJNS Submission (3)/figures/nn_model.tex <==
\begin{figurehere}
\centering
\includegraphics[width=.95\columnwidth]{images/NN_model.png}
\caption{The structure of the neural network. These were applied in an ensemble model, so the outputs of 300 independently-trained neural networks were averaged in a cross-validation scheme.}
\label{fig:nn_model}
\end{figurehere}

==> IJNS Submission (3)/figures/rest_or_task_fig.tex <==
\begin{figure*}
\centering
\raisebox{40ex}{\fontfamily{qhv}{\fontsize{30}{100}{\textbf{A}}}}
\includegraphics[width=0.6\linewidth]{images/wc_all_rest_or_task_top_100_collection_random.png}
\raisebox{40ex}{\fontfamily{qhv}{\fontsize{30}{100}{\textbf{B}}}}\includegraphics[width=0.45\linewidth]{images/diversity_index_covars_rest_or_task.png}
\raisebox{40ex}{\fontfamily{qhv}{\fontsize{30}{100}{\textbf{C}}}}\includegraphics[width=0.40\linewidth]{images/rest_or_task_auroc_plot.png}
\caption{Results for resting-state/task classification. (A) The 100 strongest connections of the mean class activation maps, with the maximum value taken across wavelet correlations. (B) The distribution of the diversity index of maximal activations across all filters over 300 models, showing how much filters in general were dedicated to particular phenotypes. (C) The overall classification AUROC and the AUROC of individual data collections in the model, showing the overall and relative success of the model.}
\label{fig:rest_or_task_fig}
\end{figure*}

==> IJNS Submission (3)/tables/table1.tex <==
\begin{table*}
\tbl{Average populations present for successfully-preprocessed datasets. Some datasets were not labeled with respect to one or more covariates, so counts may not sum to the listed total. \label{tab:table1}}
{\begin{tabular}{@{}lrrrrrrrrrrr@{}}
\toprule
& & & & & Age & & & & Sex & & Disorders \\
Collection & Subjs & Conns & Rest & Task & Min & Max & Mean & Stddev & F & M & Autism \\ \colrule
1000 FC & 764 & 764 & 764 & 0 & 7.88 & 85.00 & 25.76 & 10.18 & 443 & 321 & 0 \\
ABCD & 1319 & 9205 & 4043 & 5162 & 0.42 & 11.08 & 10.08 & 0.65 & 4339 & 4866 & 113 \\
Abide & 193 & 193 & 193 & 0 & 9.00 & 50.00 & 17.81 & 6.69 & 21 & 172 & 94 \\
Abide II & 720 & 761 & 761 & 0 & 5.22 & 55.00 & 14.44 & 7.45 & 174 & 587 & 375 \\
ADNI & 141 & 261 & 261 & 0 & 56.00 & 95.00 & 73.57 & 7.32 & 146 & 115 & 0 \\
BioBank & 11811 & 16970 & 9937 & 7033 & 40.00 & 70.00 & 55.23 & 7.51 & 8752 & 8218 & 8 \\
ICBM & 112 & 381 & 29 & 352 & 19.00 & 74.00 & 43.53 & 14.83 & 188 & 193 & 0 \\
NDAR & 1123 & 8569 & 5952 & 2617 & 0.25 & 55.83 & 18.65 & 7.82 & 4165 & 4404 & 994 \\
Open fMRI & 1443 & 6655 & 1169 & 5486 & 5.89 & 78.00 & 27.22 & 10.40 & 2768 & 3133 & 127 \\
All & 17614 & 43838 & 23109 & 20650 & 0.25 & 95.00 & 33.05 & 20.68 & 20996 & 22009 & 1711 \\
\botrule
\end{tabular}}
\end{table*}

==> IJNS Submission (3)/tables/table2.tex <==
\begin{tablehere}
\tbl{The ensemble and averaged AUROCS and accuracies for 300 models.\label{tab:table2}}
{\begin{tabular}{@{}llll@{}}
\toprule
 & Autism & Gender & Rest v Task \\ \colrule
%Mean AUROC & 0.6586 & 0.7446 & 0.8450 \\
%AUROC Stddev & 0.0229 & 0.0207 & 0.0296 \\
%Peak AUROC & 0.7201 & 0.8032 & 0.892 \\
%Mean Acc. & 63.99\% & 68.74\% & 77.09\% \\
%Acc. Stddev & 2.05 & 2.03 & 3.56 \\
%Peak Acc. & 69.11\% & 73.45\% & 83.56\% \\
Ensemble AUROC & 0.6774 & 0.7680 & 0.9222 \\
Ensemble Acc. & 67.0253\% & 69.7063\% & 85.1996\% \\
Average AUROC & 0.6133 & 0.6858 & 0.9231 \\
Average Acc. & 57.1150\% & 63.3398\% & 84.3153\% \\

\botrule
\end{tabular}}
\end{tablehere}

==> figures/collection_distributions.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=0.9\linewidth]{images/all_collection_dist.png}
\caption{The effects of collection-based class balancing on the total degree distributions of wavelet correlation matrices. Note that data is re-scaled to have values in between 0 and 1, and the distributions are normalized for comparisons to have a total area of 1.}
\label{fig:collection_distribution}
\end{center}
\end{figure*}
